Exact Algorithms via Monotone Local Search

We give a new general approach for designing exact exponential-time algorithms for subset problems. In a subset problem the input implicitly describes a family of sets over a universe of size n and the task is to determine whether the family contains at least one set. Our approach is based on "monotone local search", where the goal is to extend a partial solution to a solution by adding as few elements as possible. More formally, in the extension problem we are also given as input a subset X of the universe and an integer k. The task is to determine whether one can add at most k elements to X to obtain a set in the (implicitly defined) family. Our main result is that an O*(c^k) time algorithm for the extension problem immediately yields a randomized algorithm for finding a solution of any size with running time O*((2-1/c)^n). In many cases, the extension problem can be reduced to simply finding a solution of size at most k. Furthermore, efficient algorithms for finding small solutions have been extensively studied in the field of parameterized algorithms. Directly applying these algorithms, our theorem yields in one stroke significant improvements over the best known exponential-time algorithms for several well-studied problems, including d-Hitting Set, Feedback Vertex Set, Node Unique Label Cover, and Weighted d-SAT. Our results demonstrate an interesting and very concrete connection between parameterized algorithms and exact exponential-time algorithms. We also show how to derandomize our algorithms at the cost of a subexponential multiplicative factor in the running time. Our derandomization is based on an efficient construction of a new pseudo-random object that might be of independent interest. Finally, we extend our methods to establish new combinatorial upper bounds and develop enumeration algorithms.

==> weighted.tex <==
\newcommand{\wphisub}{\textsc{Weighted} \phisub}
\newcommand{\wphiext}{\textsc{Weighted} \phiext}
\newcommand{\pwphiext}{\textsc{Permissive Weighted} \phiext}
%\newcommand{\pphiext}{\textsc{Permissive} \phiext}

%\subsection{Weighted problems}

Let us now discuss how our approach can be used for weighted problems.

The \phisub\ problem can naturally encode weighted problems: the instance $I$ has some weights associated to the elements of $U_I$ and a target weight $W$, and $\mathcal{F}_I$ contains only sets with weight at most (or at least) $W$.

Recall, though, that the \phiext\ problem is to decide whether, for an instance $I$, a set $X\subseteq U_I$, and an integer $k$, there exists a subset $S \subseteq U_I \setminus X$ such that $S \cup X \in \mathcal{F}_I$ and $|S| \le k$. That means that the FPT subroutine needs to be able to decide whether there exists such a set $S$ with size at most $k$ and weight at most $W'=W-w(X)$. Importantly, we require the running time to be $c^k \bitsize^{\Oh(1)}$, whereas the running time is often upper bounded in terms of $W'$ for weighted problems.

In \cite{AgrawalLKS15}, such a variant of \textsc{Weighted Feedback Vertex Set} was considered, and an algorithm was presented finding a feedback vertex set with size at most $k$ and weight at most $W$, if one exists, in time $3.1681^k n^{\Oh(1)}$.


% outline how our approach can be used for weighted problems.
%A \emph{weighted set system} $(U, {\cal F}, w)$ is composed of a set system $(U, {\cal F})$ and a weight function $w: U\rightarrow \mathbb{N}_0$ equipping each element of $U$ with a non-negative integer. Similar to an implicit set system, an \emph{implicit weighted set system} is a function $\Phi$ that takes as input a string $I \in \{0,1\}^*$ and outputs a weighted set system $(U_I, {\cal F}_I, w)$.
%We refer to the string $I$ as a \emph{weighted instance}, and to $m=n+w_{\text{enc}}$ as the {\em size} of the instance, where $n=|U_I|$ and $w_{\text{enc}} = \max_{e\in S} \{\lceil \log_2 w(e) \rceil\}$.
%The implicit weighted set system $\Phi$ is said to be {\em polynomial time computable} if (a) there exists a polynomial time algorithm that given $I$ produces $U_I$ and $w$, and (b) there exists a polynomial time algorithm that given $I$, $U_I$ and a subset $S$ of $U_I$ determines whether $S \in{\cal F}_I$.
%% Observe that the size of ${\cal F}_I$ can be exponential in $|I|$ and in $|U_I|$. Therefore the fact that an implicit set system $\Phi$ is polynomial time computable does not yield a polynomial time algorithm to produce ${\cal F}_I$ from $I$.
%We also note that all implicit weighted set systems discussed in this paper are polynomial time computable.
%
%\defproblem{\wphisub}{A weighted instance $I$}{Find a minimum weight set $S \in {\cal F}_I$.}
%\medskip
%
%The \emph{weight} of a set $S\subseteq U_I$ is the sum of the weights of its elements, i.e., $w(S) = \sum_{e\in S} w(e)$.
%We observe that negative and rational weights can be accommodated by appropriate scaling.
%
%We will demonstrate how single-exponential parameterized algorithms for the following problem with parameter $k$ can be turned into algorithms for \wphisub.
%
%\defproblem{\wphiext}{A weighted instance $I$, a set $X \subseteq U_I$, an integer $k$, and an integer $W$.}
%{Does there exists a subset $S \subseteq (U_I \setminus X)$ such that $S \cup X \in {\cal F}_I$, $w(S)\le W$, and $|S| \leq k$?}
%
%\begin{lemma}\label{lem:weighted}
% If there exists an algorithm for \wphiext{} with running time $c^km^{\Oh(1)}$ then there exists a randomized algorithm for \wphisub\ with running time $(2-\frac{1}{c})^{n}m^{\Oh(1)}$.
% and a deterministic algorithm for \wphisub\ with running time $(2-\frac{1}{c})^{n}2^{o(n)}m^{\Oh(1)}$.
%\end{lemma}
%\begin{proof}
%% Let $\mathcal{B}$ be an algorithm for \wphiext{} that solves instances $(I,X,k,W)$ in time $c^km^{\Oh(1)}$.
% To design algorithms for \wphisub\ with the claimed running times, proceed as follows.
% First, compute $U_I$ and $w$ in polynomial time.
% Let $w_{\text{max}} = \max_{e\in U_I} \{w(e)\}$ denote the maximum weight of an element in $U_I$.
% Using binary search between values $0$ and $n\cdot w_{\text{max}}$ for $W$, we will design an algorithm to determine whether $I$ has a set $S\in \mathcal{F}_I$ of weight at most $W$. Solving this problem $m^{\Oh(1)}$ times and using standard self reducibility gives an algorithm for \wphisub\ at the cost of a polynomial overhead in the instance size.
% To determine whether $I$ has a set $S\in \mathcal{F}_I$ of weight at most $W$, we observe that solving \wphisub\ for $I$ is equivalent to solving \phisub for an instance $I'$ that is equivalent to $I$, except that $F_{I'}$ contains no set with weight more than $W$. Similarly, an instance for \wphiext\ can be cast as an instance for \phiext by excluding subsets from $\mathcal{F}_I$ with weight greater than $W$.
% The lemma now follows from Theorems \ref{thm:main1} and \ref{thm:main2}.
%\end{proof}


Shachnai and Zehavi \cite{ShachnaiZ15} gave a $2.168^k \bitsize^{\Oh(1)}$ time algorithm for permissive variants of \textsc{Weighted 3-Hitting Set}: if the instance has a hitting set of weight at most $W$ and size at most $k$, the algorithm returns such a hitting set (\yes), else if it has a hitting set of weight at most $W$ it returns such a hitting set (\yes) or \no, and otherwise it returns \no.
Moreover, by Fomin et al.'s iterative compression approach \cite{FominGKLS10}, the algorithm of Shachnai and Meirav can be extended to $d\ge 4$,
giving algorithms with running times $O((d-0.832)^k \bitsize^{\Oh(1)})$.
Using Lemma \ref{thm:permissive} this gives algorithms for \textsc{Weighted} $d$-\textsc{Hitting Set} with running time $(2-\frac{1}{d-0.832})^n m^{\Oh(1)}$.

\todo[inline]{Add: Weighted $d$-Sat}



% DONE \todo[inline]{check running time for \textsc{Weighted Feedback Vertex Set}  $3.619^k$   \cite{AgrawalLKS15}}


